Cross-Link Channel Prediction for Massive IoT Networks

Tomorrow's massive-scale IoT sensor networks are poised to drive uplink traffic demand, especially in areas of dense deployment. To meet this demand, however, network designers leverage tools that often require accurate estimates of Channel State Information (CSI), which incurs a high overhead and thus reduces network throughput. Furthermore, the overhead generally scales with the number of clients, and so is of special concern in such massive IoT sensor networks. While prior work has used transmissions over one frequency band to predict the channel of another frequency band on the same link, this paper takes the next step in the effort to reduce CSI overhead: predict the CSI of a nearby but distinct link. We propose Cross-Link Channel Prediction (CLCP), a technique that leverages multi-view representation learning to predict the channel response of a large number of users, thereby reducing channel estimation overhead further than previously possible. CLCP's design is highly practical, exploiting channel estimates obtained from existing transmissions instead of dedicated channel sounding or extra pilot signals. We have implemented CLCP for two different Wi-Fi versions, namely 802.11n and 802.11ax, the latter being the leading candidate for future IoT networks. We evaluate CLCP in two large-scale indoor scenarios involving both line-of-sight and non-line-of-sight transmissions with up to 144 different 802.11ax users. Moreover, we measure its performance with four different channel bandwidths, from 20 MHz up to 160 MHz. Our results show that CLCP provides a 2x throughput gain over baseline 802.11ax and a 30 percent throughput gain over existing cross-band prediction algorithms.

==> defs.tex <==
\usepackage[sf,bf,medium]{titlesec}
\usepackage{calc,booktabs,color,colortbl,multirow}
% \usepackage{graphicx}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}

\special{papersize=8.5in,11in}
\setlength{\pdfpagewidth}{8.5in}
\setlength{\pdfpageheight}{11in}

\definecolor{Gray}{gray}{0.9}
\definecolor{LightGreen}{rgb}{0.88,1,0.88}
\definecolor{LightYellow}{rgb}{1,1,0.8}
\definecolor{LightOrange}{rgb}{1,0.85,0.8}
\definecolor{LightRed}{rgb}{1,0.80,0.80}

\setcounter{tocdepth}{4}
\setcounter{secnumdepth}{4}

\pdfoptionpdfminorversion=6

\newcommand{\figref}[1]{Figure~\ref{#1}}

\newcommand{\longnamenoprefix}{MLWiNS: Large-Scale Wireless Cross-Link Channel Prediction (CLCP)\xspace}
\newcommand{\shortname}{CLCP}
\newcommand{\shortnameposs}{CLCP's}
\newcommand{\longname}{\longnamenoprefix\xspace}
\newcommand{\shortnames}{\shortnameposs}
\newcommand{\systemname}{\shortname}
\newcommand{\systemnames}{\shortnameposs}

\newcommand{\clcp}{CLCP}
\newcommand{\clcps}{CLCP's}
\newcommand{\cljo}{CLJO}
\newcommand{\cljos}{CLJO's}

% Six lines per inch (NSF maximum): 0.883
\renewcommand{\baselinestretch}{1.000}
\setlength{\parskip}{2pt plus 1pt minus 0pt}

\titleformat{\section}[hang]
  {\normalfont\large\sffamily\bfseries}
  {\noindent\large$\blacksquare$\enspace\thesection}
  {1pc}
  {\large\thispagestyle{fancy}}

\titleformat{name=\section,numberless}[hang]
 {\normalfont\large\sffamily\bfseries}
 {\noindent\large$\blacksquare$\enspace}
 {0.5pc}
 {\large\thispagestyle{fancy}}

\titleformat{\subsection}[hang]
  {\normalfont\large\sffamily\bfseries}
  {\thesubsection}{1em}{}

\titleformat{\subsubsection}
  {\normalfont\large\sffamily\bfseries}
  {\thesubsubsection}{1em}{}

\titlelabel{\thetitle\enskip}
\titlespacing*{\section}{-15.39pt}{*4}{4pt}
\titlespacing*{\subsection}{0pt}{*3}{2pt}
\titlespacing*{\subsubsection}{0pt}{*2}{2pt}
\titlespacing*{\paragraph}{0pt}{4pt plus 2pt minus 2pt}{1.25ex}
\titlespacing*{\subparagraph}{0pt}{4pt plus 2pt minus 2pt}{1.25ex}

\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\setlength{\textfloatsep}{10pt plus 2pt minus 2pt} 
\setlength{\intextsep}{10pt plus 2pt minus 2pt}

% \setitemize{itemsep=2pt,topsep=4pt,parsep=2pt,partopsep=0pt,leftmargin=1.5em}
% \setenumerate{itemsep=2pt,topsep=2pt,parsep=1pt,partopsep=0pt,leftmargin=1.5em}
% \setlist{itemsep=2pt,parsep=2pt}

\newcommand{\eg}{{\itshape e.g.,\@}\xspace}
\newcommand{\ie}{{\itshape i.e.,\@}\xspace}
\newcommand{\ca}{{\itshape ca.\@}\xspace}
\newcommand{\outcome}{{\sffamily\bfseries {\scriptsize 
$\blacksquare$}~Assessment criterion---}\xspace}
\newcommand{\outcomes}{{\sffamily\bfseries {\scriptsize
$\blacksquare$}~Assessment criteria---}\xspace}

\hyphenation{E-SNR PR-ESS MI-MO of-dm end-points CO-PA FI-CA back-scat-ter WA-RP beam-width}

\newcommand{\todo}[1]{\textcolor{red}{{\bfseries #1}}}

\newcommand{\note}[2]{\textbf{\textcolor{#1}{#2}}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\heading}[1]{\vspace{2pt plus 2pt minus 2pt}\noindent{\sffamily\bfseries #1}}
\newcommand{\parabreak}{\vspace*{1.00ex minus 0.25ex}\noindent}
\newcommand{\parahead}[1]{\vspace*{1ex plus 0ex minus 0.25ex}\noindent{}{\bfseries #1}}


\makeatletter
\def\cleardoublepage{\clearpage\if@twoside%
    \ifodd\c@page\else
    \vspace*{\fill}
    \hfill
    \begin{center}
    This page intentionally left blank.
    \end{center}
    \vspace{\fill}
    \thispagestyle{empty}
    \newpage
    \if@twocolumn\hbox{}\newpage\fi\fi\fi
}
\makeatother

\renewcommand{\theparagraph}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}(\alph{paragraph})}
\renewcommand{\thepage}{\arabic{page}}


==> scheduling.tex <==
\section{AX-SRA Algorithm}
\label{s:sra}

The problem of user grouping and resource allocation in 802.11ax 
is highly challenging
as it combines both MU\hyp{}MIMO and OFDMA functionality. 
%Thus, suboptimal user scheduling with a massive-IoT system 
%not only incurs significant feedback overhead but 
%also induces excessive computational overhead, and MAC\hyp{}layer overhead. 
Here, we solve the problem in the context of 802.11ax.
% In general, the well-known scheduling algorithms in LTE leverage 
% (1) max sum rate, (2) proportional fair. 
% In this paper, we propose a scheduling algorithm that integrates 
% the max sum rate and proportional fair scheduler using the channel condition and buffer status. 

\begin{figure}[t]
\includegraphics[width=0.92\linewidth]{figures/ofdma_alloc.pdf}
\caption{Uplink trigger-based OFDMA with four user groups with an equal amount of data $D$, $20 MHz$ bandwidth, $p_{j}=\left \{ RU(2,0),~RU(2,1),~RU(3,e),~RU(1,1) \right \}$ and $u_{j} = \left \{\left \{ 1 \right \}, \left \{ 2 \right \}, \left \{ 3 \right \}, \left \{ k \right \} \right \}$, and scheduling duration $T_{s}$. }
\label{f:protocol:ofdma_allocation}
\vspace{-4pt}
\end{figure}

\parahead{Problem Formulation.}
% Consider 802.11ax setting with AP and user set $U = {1,2,\dots,N}$ equipped with $M_{AP}$ and $M_{STA}$ antennas, respectively. 
With up-to-date CSI and BSR of all users, we can formulate the scheduling problem as the following optimization task. 
Each time unit, the scheduler allocates RUs to some clients in order to maximize 
% $U = \sum^{N}_{i=1} \sum^{M}_{j=1} x^{j}_{i} \lambda^{j}_{i}$
% where $\lambda^{j}_{i}$ denotes the utility value for STA $i$ in $j$th RU. 
% Given a RU configuration $g \in G$, the optimization goal is:
    % &max (U_{g}) = max (\sum^{N}_{i=1} \sum^{M}_{j=1} x^{j}_{i} \lambda^{j}_{i}) \\
    % &st \sum^{N}_{i=1} x^{j}_{i} \leq 1, \forall j \in [1,M],
    % \sum^{M}_{j=1}x^{j}_{i} \leq 1, \forall i \in [1,N]   
% \begin{equation}
% \label{eq:2}
% \begin{aligned}
%     &max (F) = max_{g\in G}R_{ZFBF}(g) \\
%     &st \sum^{N}_{i=1} x^{j}_{i} \leq 1, \forall j \in [1,M],
%     \sum^{M}_{j=1}x^{j}_{i} \leq 1, \forall i \in [1,N] 
% \end{aligned}
% \end{equation}
zero\hyp{}forcing beamforming (ZFBF) capacity, which we compute by 
summing the achieved rates at each subcarrier $s$, that is
$R_{\mathrm{ZFBF}}(RU(l,i)) = \sum_{s\in RU(l,i)} R_{\mathrm{ZFBF}}(s)$. Then, the
ZFBF capacity of the complete user schedule $g$ is written as:
\begin{equation}
\vspace{-2pt}
\begin{aligned}
    % R_{ZFBF}(g) = 
    \sum_{j}R_{\mathrm{ZFBF}}(p_{j},u_{j}) = 
    \sum_{j}\sum_{s\in p_{j}}\sum_{u\in u_{j}}\log_{2}(1+P_{u,s})
\end{aligned}
\end{equation}
where $P_{u,s}$ denotes the transmit power for user $u$ and subcarrier $s$. 
Finally, the optimization objective becomes:
\begin{equation}
\vspace{-2pt}
\begin{aligned}
    &U = 
    \max_{g \in G} R_{\mathrm{ZFBF}}(g) \\
    &s.t. ~0 \leq \sum_{j} c_{j,u} \leq 1,~1 \leq \sum_{u} c_{j,u} \leq \left \lfloor N_{T}/N_{R} \right \rfloor
\end{aligned}
\end{equation}
where $c_{j,k} \in \left \{ 0,1 \right \}$ indicates if user or user group $k$ is allocated on the $j$th RU, $G$ is the set of all possible user schedules, and $N_{T}$ and $N_{R}$ denote the number of transmitter and receiver antenna, respectively. Last two equations simply define the constraints that unlike LTE that enables the allocation of multiple resource blocks (RB) to a single user, 802.11ax restricts a single RU to each user, and the number of users allocated on RU is between $1$ and
$\left \lfloor N_{T}/N_{R} \right \rfloor$.

Since in 802.11ax
the transmission duration $T_{s}$ must
start and end at the same time for all the users in the same 
OFDMA timeslot, users with insufficient
data append null data (\textit{i.e.} padding) to match the time duration.
For instance, assume the optimal user schedule 
$g_{\mathrm{opt}}=\arg \max_{g \in G}R_{\mathrm{ZFBF}}(g)$ in
Fig.~\ref{f:protocol:ofdma_allocation}. According to BSRs, the users assigned to RUs have 
an equal amount of data to simultaneously send. Due to variable RU sizes (two with $52$-tone RU, 
one with $26$-tone RU, and one with $106$-tone RU), the user group $u_{j}$ assigned to RU of 
a different level $l$ consists of different transmission time $T_{j}$. However, in 
order to end transmission of the users at the same time, the users with insufficient data 
transmit null data
%$T_{null,j} = \max_{j \in g}\left\{T_{j}\right\} - T_{j} \forall j$. 
which significantly degrades capacity and energy efficiency.
Dividing the scheduled packet into multiple smaller packets based on the minimum 
transmission duration among the users (\textit{e.g.} $T_{k}$ in 
Fig.~\ref{f:protocol:ofdma_allocation}) can minimize the padding, but 
increasing the number of packet leads to high medium contention overhead. 
Thus, to optimize the balance between MAC layer overhead (due to padding) and 
medium contention overhead (due to a large number of packets), we consider 
buffer status in the scheduling algorithm in addition to channel capacity.
\begin{algorithm}[t]
% \SetAlgoLined
\noindent 
\begin{algorithmic}[1] % enter the algorithmic environment
\Require 
    \Statex The up-to-date $CSI_{u}$ and $BSR_{u}$ $\forall u \in U$
\While{$\sum_{u}^{U} BSR_{u} > 0$}
    \State $MCS_{u}$ = \textbf{Rate-Adaptation}($CSI_{u}$) $\forall u \in U$
    \If{OFDMA}
        % Compute $MCS_{u}$ given $eSNR_{u}$ 
        \State Compute $R_{u} = BSR_{u}/T_{MaxTime}$ $\forall u \in U$
        \State Find $R_{RU(0)}, \dots, R_{RU(L)}$ given $MCS_{u}$ $\forall u \in U$
        \State $U_{l} \cap \left \{ u \right \}$ where  $l \geq \operatorname*{argmin}_{l \in L} \left \| R_{RU(l)} - R_{u} \right \| $
        \State $g_{opt} = \textbf{Divide-Conquer}(U, CSI, 0,0)$
    \Else
        \State $g_{opt} = \textbf{User-Grouping}(U, CSI,0,0)$
    \EndIf
    % \State Allocate $g_{RA} = g_{RU}-g_{SA}$ RUs for random access
    \While{empty $RU$ in $g_{opt}$}
        \State Pop $U_{l}$ if empty  $\forall l \in L$
        \State $g_{opt} = \textbf{Divide-Conquer}(U, CSI,0,0)$
    \EndWhile
    \State Set $T_{s} = max(min_{k \in g}(T_{k}), T_{MinTime})$
    % \If{Uplink}
    \State Transmit trigger frame
    % \EndIf
    \State Receive \text{scheduled-packet}
    \State $BSR_{u} = BSR_{u} - \text{Scheduled-Packet } \forall u \in g_{SA}$
    % \State Update $BSR_{u}~\forall u \in U$
    % \State 
\EndWhile
 \caption{ax-SRA algorithm}
 \label{alg:general}
 \end{algorithmic} % enter the algorithmic environment
\end{algorithm}

\parahead{ax-SRA algorithm.}
%  the AP first sends a TF which
% now only indicates the ID of the group (i.e, the IDs of
% the scheduled users), and the dedicated sub-channel to each
% scheduled user. After receiving the TF, each user sends its
% buffer status (BS) information within the BS frame (i.e.,
% Qk(t)) by using its dedicated sub-channel. Also, the AP uses
% the BS frame to estimate the uplink transmission rate of user k
% (i.e., Rk(t)). Finally, the AP has both queue size and channel
% state information of each scheduled user at that time, and
% can determine the optimal scheduling duration denoted by $T_{s}$
Algorithm~\ref{alg:general} summarizes ax-SRA, which 
consists of five major steps:
\textbf{(1)} find a proper MCS index for each user based on the acquired\fshyp{}predicted 
full\hyp{}bandwidth channel information, \textbf{(2)} assign the clients into $L+1$ 
user pool groups (\textit{e.g.} four groups for $20$~MHz
as shown in Fig.~\ref{f:protocol:ru}) according to 
each user's MCS index and BSR, \textbf{(3)} execute a modified divide\hyp{}conquer 
(DQ) algorithm with CSIs and user pools determined in step $2$, 
\textbf{(4)} if the schedule result in Step~$3$ contains RU with no assigned user, 
rearrange the users in the user pool groups from Step~$2$ and re\hyp{}execute 
Step~$3$, and \textbf{(5)} enforce the packet duration to the minimum scheduling duration among all scheduled users.

For the first step, we conduct effective SNR (ESNR)\hyp{}based
rate adaptation~\cite{halperin2010predictable}
using a full-bandwidth channel. Specifically, we select an appropriate MCS index 
by comparing the channel's ESNR against the pre\hyp{}determined threshold 
that allows successfully delivery of the packets.
This pre-determined threshold is set to the SNR value that guarantees successful packet delivery (\textit{i.e.} $100\%$ packet reception rate (PRR))
% based on the following observation on the OFDMA packet: 
because according to our simulation result,
larger RUs achieve higher PRR than smaller RUs when SNR is relatively high for every MCS index
in frequency-selective multipath environment.
% while larger RUs provide higher PRR compared to smaller RUs when SNR is moderately high. 
As seen in Fig.~\ref{f:protocol:packet_delivery},
% shows the packet delivery for each RUs in frequency-selective multipath environment. 
at SNR in which full-bandwidth RU achieves $100\%$ PRR, all smaller RUs attain PRR lower than $100\%$ but above $90\%$.
% , even for the smallest RU with $26$ subcarriers. 
% This observation is shown for every MCS index. 
If the PRR gap between full-bandwidth RU and smallest RU is larger than $10\%$ due to a highly frequency-selective fading channel, 
we increment threshold to the value in which the gap near $10\%$.

% \todo{editing...}
To minimize discrepancy between the buffer capacity of $j$th RU and data size of user $u_{j}$, 
we create the user pool groups associated with the level of RU, which is an indication of RU size (\textit{e.g.} recall Fig.~\ref{f:protocol:ru} depicting that RU at level $L$ is $26$-tone RU, and RU at level $0$ is $242$-tone RU for $20$Mhz). 
When allocating resources, each RU selects the users\fshyp{}user groups within the user pool group associated with its corresponding level. 
The purpose is to prevent against assigning the low data-rate users into large RU, avoiding both the addition of padding and unnecessary MIMO execution for small data. 
However, to increase user scheduling opportunities, we want to allow high data-rate users for small RUs. 
% We will discuss in detail when describing the modified DQ algorithm.
To create these user pools, we need to assign the users into $L+1$ user pool groups $U_{0},\dots,U_{L}$ using BSR and selected MCS index. 
Specifically, we first compute the data-rate $R_{u}$ for each user $u$ via dividing the length of its data indicated in $BSR$ by the maximum allowed duration of a packet $T_{MaxTime}$, which is $5.484 ms$~\cite{802.11ax-wc16}. 
Then, we compare the calculated data-rate $R_{u}$ with predefined
% $L+1$ 
PHY rates~\cite{802.11ax-wc16} supported by RUs of every level $R_{RU(0)},\dots,R_{RU(L)}$
% , predefined in the 802.11ax rate table~\cite{802.11ax-wc16}, 
at the selected MCS index. 
Specifically,  we find the level $l$ in which among all levels whose $R_{RU}$ is greater than $R_{u}$, $R_{RU}$ is closest to the $R_{u}$. With this level $l$, we assign the users to all user pool groups whose level is greater than or equal to $l$.
% ($l = \operatorname*{argmin} \left \| R_{RU(l)} - R_{u} \right \|$). 
% We assign 
% of the user pool groups $U_{l}$ for all level $l$ in which  $R_{RU(l)}$ is less than $R_{u}$. 
% If there are multiple groups whose $R_{RU(l)} < R_{u}$, we assign $u$ into all of these groups. 
% where among $R_{u}$ less than $R_{RU(l)}$, $l = \operatorname*{argmin} \left \| R_{RU(l)} - R_{u} \right \|$. 
For users $u$ with $R_{u}$ greater than $R_{RU(0)}$, we assign $u$ to all user pool groups. 

\begin{figure}[t]
\vspace{-5pt}
\includegraphics[width=0.9\linewidth]{figures/mcs_white.pdf}
\caption{802.11ax packet delivery for each RU in 20MHz bandwidth, simulated with maximum delay of $390$ ns.}
\vspace{-4pt}
\label{f:protocol:packet_delivery}
\end{figure}

% \begin{table}[t]
% \centering
% \scalebox{0.75}{\begin{tabular}{ |p{0.4cm}|p{2.2cm}||p{1cm}|p{1cm}|p{1cm}|p{1cm}|  }
% %  \hline
% %  \multicolumn{6}{|c|}{Data rate $D_{RU}$ of 20MHz channel in Mbps} \\
%   \hline
%  \multicolumn{2}{|c||}{MCS} & $R_{RU(3)}$& $R_{RU(2)}$& $R_{RU(1)}$& $R_{RU(0)}$\\
%  \hline
%  0 & BPSK, 1/2       &0.8 & 1.5 & 3.2 & 7.3\\
%  1 & QPSK, 1/2       &1.5 & 3.0 & 6.4 & 14.6\\
%  2 & QPSK, 3/4       &2.3 & 4.5 & 9.6 & 21.0\\
%  3 & 16-QAM, 1/2     &3.0 & 6.0 & 12.8 & 29.3\\
%  4 & 16-QAM, 3/4     &4.5 & 9.0 & 19.1 & 43.9\\
%  5 & 64-QAM, 2/3     &6.0 & 12.0 & 25.5 & 58.5\\
%  6 & 64-QAM, 3/4     &6.8 & 13.5 & 28.7 & 65.8\\
%  7 & 64-QAM, 5/6     &7.5 & 15.0 & 31.9 & 73.1\\
%  8 & 256-QAM, 3/4    &9.0 & 18.0 & 38.3 & 87.8\\
%  9 & 256-QAM, 5/6    &10.0 & 20.0 & 42.5 & 97.5\\
%  10 & 1024-QAM, 3/4  & \_ & \_ & \_ & 109.7\\
%  11 & 1024-QAM, 5/6  & \_ & \_ & \_ & 121.9\\
%  \hline
% \end{tabular}}
% \caption{Maximum theoretical throughput in 802.11ax with $20MHz$ bandwidth ($L=3$).}
% \label{table:rates}
% \vspace{-4pt}
% \end{table}


\begin{figure*}[h]
\begin{subfigure}[b]{0.265\linewidth}
\includegraphics[width=\linewidth]{figures/LOSRoom_small2.pdf}
\caption{LOS testbed.}
\label{f:testbed:loc}
\end{subfigure}
% \hfill
\begin{subfigure}[b]{0.55\linewidth}
\includegraphics[width=\linewidth]{figures/NLOSRoom_small2.pdf}
\caption{NLOS testbed.}
\label{f:testbed:room}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.12\linewidth}
\includegraphics[width=\linewidth]{figures/hardware.png}
\caption{Hardware.}
\label{f:testbed:hardware}
\end{subfigure}
\vspace{-5pt}
\caption{\clcp{} preliminary experimental testbed 
floor plans (radios-$\bigcirc$, moving reflectors-$\triangle$) and radio hardware.}
\label{f:testbed}
\vspace{-5pt}
\end{figure*}

% However, the size of the search space still increases exponentially with the number of users and RU granularity.
We then leverage the DQ algorithm~\cite{wang2018scheduling} (see Appendix for details) with three modifications. 
To briefly explain this algorithm, given the RU abstraction shown in Fig.~\ref{f:protocol:ru}, $RU(l,i)$ splits into $RU(l+1,2i)$ and $RU(l+1,2i+1)$ in the divide step, with each RU at level $l+1$ treated as a subproblem that is independently solved. 
Let the optimal user schedules on $RU(l+1,2i)$ and $RU(l+1,2i+1)$ be $g_{opt}(l+1,2i)$ and $g_{opt}(l+1,2i+1)$ that maximizes the sum rate of ZFBF capacity. In the merge step, $g_{opt}(l+1,2i)$ and $g_{opt}(l+1,2i+1)$ merges into $g_m(l,i)$.
At $RU(l,i)$, the algorithm calculates the best schedule $g_{s}(l,i)$. 
Then, the optimal schedule $g_{opt}(l,i)$ is the one that provides higher ZFBF capacity between $g_{s}(l,i)$ and $g_{m}(l,i)$.
Our first modification here is that $RU$ at level $l$ selects the users within its user pool group $U_{l}$.
Secondly, since 11ax restricts one RU per each user, ax-SRA removes the user $u$ selected in $g_{opt}(l,i)$ from $U_{l}$ so that $u$ is not considered for other RUs. 
Lastly, since the original DQ algorithm does not consider extra $RU(l,e)$ (see Fig.~\ref{f:protocol:ru}), we add constraint that in the merge step at level $L-3$, $g_{opt}(L-2,2i)$, $g_{opt}(L,e)$, and $g_{opt}(L-2,2i+1)$ merges into $g_m(L-3,i)$. 
For RUs larger than $106$ subcarriers, we use greedy user selection algorithm for MU-MIMO.

% \todo{Additional rank up algorithm not yet addressed.}
Once the modified DQ algorithm finalizes $g_{opt}$, ax-SRA checks if $g_{opt}$ contains RU with no user, which is due to a small number of user candidates, especially in the user pool group with lower level. Thus, we rearrange the list of user pool groups by removing the empty user pool groups and lowering the level of existing groups. For example, if two groups are removed among four, then $U_{2}$, and $U_{3}$ becomes $U_{0}$ and $U_{1}$. Then, we re-execute the DQ algorithm. This guarantees non-empty RU by enforcing the use of larger bandwidth.
% , we assign random access $g_{RA}$. 

For each user $k \in {1, 2, \dots, K}$ at time $t$, the optimal transmission duration $T^{*}_{s}(t)$ that maximizes the total throughput is equal to $T_{min}(t)$ among all users. 
% i.e., $T^{*}_{s}(t) = T_{min}(t)$
Therefore we enforce $T_{s} = max(min_{k \in g_{opt}}(T_{k}), T_{MinTime})$ with finalized $g_{opt}$. 
This operation naturally prevents the addition of padding for the the schedules that assigned high data-rate users assigned to small RUs. Then the AP transmits the trigger frame, and
% \todo{model on how this is done.}
% In downlink, the AP transmits the scheduled packets while
% In uplink, the AP sends a TF containing both common information (e.g. transmission duration) and information specific per STA (e.g. allocated RU, MCS, frequency and time synchronization). The scheduled STAs respond according to the mode defined in the TF. 
once the AP receives the scheduled packet, ax-SRA repeats itself until no more data is left in BSRs. 
% $RU_{26} = RU_{52}*(1/2) = RU_{106}*(1/4) = RU_{242}*(1/9)$
% \begin{equation}
% TXTIME = 20 + THE-PREAMBLE + NSYMTSYM + NMANHE-LTFTHE-LTF-SYM + TPE + SignalExtension
% \end{equation}




% Besides the first challenge of feedback overhead, 
% the second challenge of computational overhead due to 
% the tasks of optimal user selection and resource unit
% (RU) allocation remains a significant 
% problem.  As MU-MIMO capacity depends on channel correlation between
% users in a beamforming group, a poor choice of beamforming group 
% may lead to significant losses in spectral efficiency. 
% However, exhaustively searching all possible user combinations 
% is computationally infeasible, as the number of possible user groups 
% increases exponentially with base station antenna count and user count 
% \cite{shen2015sieve}.
% Furthermore, frequency\hyp{}selective channel fading 
% makes it important to select appropriate sub\hyp{}channel blocks for
% each user.  An exhaustive search would consider all possible 
% user schedules to find the optimal schedule, but 
% is impractical due to its complexity, as the size of the search space
% increases exponentially with the number of users and
% RU granularity \cite{wang2018scheduling}. 
% The overall capacity of MU-MIMO critically depends on the 
% channel correlation among the users in a beamforming group. 
% Hence, naively selecting a beamforming group may lead to
% significantly reduced data rates on concurrent transmitting links. 
% Similarly, the management and allocation of resources also impacts
% spectral efficiency. 
